Particle Flow Gaussian Sum Particle Filter

Particle flow Gaussian particle flow (PFGPF) uses an invertible particle flow to generate a proposal density. It approximates the predictive and posterior distributions as Gaussian densities. In this paper, we use bank of PFGPF filters to construct a Particle flow Gaussian sum particle filter (PFGSPF), which approximates the predictive and posterior as Gaussian mixture model. This approximation is useful in complex estimation problems where a single Gaussian approximation is not sufficient. We compare the performance of this proposed filter with PFGPF and others in challenging numerical simulations.

==> bib_file.tex <==
@inproceedings{gordon1993novel,
  title={Novel approach to nonlinear/non-{G}aussian {B}ayesian state estimation},
  author={N. Gordon and D. Salmond and A. Smith},
  booktitle={IEE Proc. F Radar Signal Process.},
  volume={140},
  number={2},
  pages={107--113},
  year={1993},
  month={Apr}
}

@ARTICLE{kotecha2003GaussianSum,
author={J. H. Kotecha and  P. M. Djuric},
journal={IEEE Trans. Signal Process.},   title={Gaussian sum particle filtering},
year={2003},
month={Oct},
volume={51},
number={10},
pages={2602--2612}
}

@article{li2019,
  title={Invertible particle-flow-based sequential {MCMC} with extension to {Gaussian} mixture noise models},
  author={Y. Li and S. Pal and M. J. Coates},
  journal={IEEE Trans. Signal Process.},
  volume={67},
  number={9},
  pages={2499--2512},
  year={2019},
  month={May}
}

@incollection{bickel2008sharp,
  title={Sharp failure rates for the bootstrap particle filter in high dimensions},
  author={P. Bickel and B. Li and T. Bengtsson},
  booktitle={Pushing the limits of contemporary statistics: Contributions in honor of Jayanta K. Ghosh},
  publisher={Institute of Mathematical Statist.},
  address={Beachwood, OH, USA},
  pages={318--329},
  year={2008}
  }
  
 @incollection{bengtsson2008curse,
  title={Curse-of-dimensionality revisited: {C}ollapse of the particle filter in very large scale systems},
  author={T. Bengtsson and P. Bickel and B. Li},
  booktitle={Probability and statistics: Essays in honor of David A. Freedman},
  publisher={Institute of Mathematical Statist.},
  address={Beachwood, OH, USA},
  pages={316--334},
  year={2008}
}

@article{snyder2008obstacles,
  title={Obstacles to high-dimensional particle filtering},
  author={C. Snyder and T. Bengtsson and P. Bickel and J. Anderson},
  journal={Mon. Weather Rev.},
  volume={136},
  number={12},
  pages={4629--4640},
  year={2008},
  month={Dec}
}

@article{arulampalam2002tutorial,
  title={A tutorial on particle filters for online nonlinear/non-{G}aussian {B}ayesian tracking},
  author={M.S. Arulampalam and S. Maskell and N. Gordon and T. Clapp},
  journal={IEEE Trans. Signal Process.},
  volume={50},
  number={2},
  pages={174--188},
  year={2002},
  month={Feb}
 }
  
 @article{pitt1999filtering,
  title={Filtering via simulation: {A}uxiliary particle filters},
  author={M. Pitt and N. Shephard},
  journal={J Ameri. Statist. Assoc.},
  volume={94},
  number={446},
  pages={590--599},
  year={1999},
  month={Jun}
  }
  
  @inproceedings{doucet2000s,
  title={{Rao-Blackwellised} particle filtering for dynamic {B}ayesian networks},
  author={A. Doucet and N. d. Freitas and K. P. Murphy and S. J. Russell},
  booktitle={Proc. Conf. Uncertainty Artif. Intell.},
  address={San Francisco, CA, USA},
  pages={176},
  year={2000}
  }
  
 @article{berzuini1997dynamic,
  title={Dynamic conditional independence models and {Markov chain Monte Carlo} methods},
  author={C. Berzuini and N. G. Best and W. R. Gilks and C. Larizza},
  journal={J. Amer. Statist. Assoc.},
  volume={92},
  number={440},
  pages={1403--1412},
  year={1997},
}

@article{gilks2001following,
  title={Following a moving target — {Monte Carlo} inference for dynamic {Bayesian} models},
  author={W. R. Gilks and C. Berzuini},
  journal={J. Roy. Statist. Soc. B,},
  volume={63},
  number={1},
  pages={127--146},
  year={2001},
  month={Jan}
}

@incollection{godsill2001improvement,
  title={Improvement strategies for {Monte Carlo} particle filters},
  author={S. Godsill and T. Clapp},
  booktitle={Sequential Monte Carlo methods in practice},
  address={New York, NY, USA},
  pages={139--158},
  year={2001}
}
  
 @incollection{musso2001improving,
  title={Improving regularised particle filters},
  author={C. Musso and N. Oudjane and F. Le Gland},
  booktitle={Sequential Monte Carlo methods in practice},
  address={New York, NY, USA},
  pages={247--271},
  year={2001}
}

@article{golightly2006bayesian,
  title={Bayesian sequential inference for nonlinear multivariate diffusions},
  author={A. Golightly and D. Wilkinson},
  journal={Statist. Comput.},
  volume={16},
  number={4},
  pages={323--338},
  year={2006},
  month={Dec}
}

@article{maroulas2012improved,
  title={Improved particle filters for multi-target tracking},
  author={V. Maroulas and P. Stinis},
  journal={J. Comput. Phys.},
  volume={231},
  number={2},
  pages={602--611},
  year={2012},
  month={Jan}
}

@inproceedings{kang2014drift,
  title={Drift homotopy particle filter for non-{Gaussian} multi-target tracking},
  author={K. Kang and V. Maroulas and I. D. Schizas},
  booktitle={Proc. Int. Conf. Inf. Fusion},
  address={Salamanca, Spain},
  pages={1--7},
  year={2014}
}

@article{brockwell2010sequentially,
  title={Sequentially interacting {Markov chain Monte Carlo} methods},
  author={A. Brockwell and P. D. Moral and A. Doucet},
  journal={Ann. Statist.},
  volume={38},
  number={6},
  pages={3387--3411},
  year={2010},
  month={Dec}
}

@article{septier2015langevin,
  title={Langevin and {Hamiltonian} based sequential {MCMC} for efficient {Bayesian} filtering in high-dimensional spaces},
  author={F. Septier and G. W. Peters},
  journal={IEEE J. Sel. Topics Signal Process.},
  volume={10},
  number={2},
  pages={312--327},
  year={2016},
  month={March}
}

@article{article,
title = {Gaussian Particle Filtering},
author = {J. Kotecha and P. Djuric},
journal = {IEEE Trans. Signal Process.},
year = {2003},
month = {Nov},
pages = {2592 - 2601},
volume = {51},
}

@inproceedings{daum2007nonlinear,
  title={Nonlinear filters with log-homotopy},
  author={F. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={6699},
  pages={423--437},
  year={2007},
  month={Sep.}
}

@inproceedings{daum2008particle,
  title={Particle flow for nonlinear filters with log-homotopy},
  author={E. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={6969},
  pages={696918},
  year={2008},
  month={Apr}
}

@inproceedings{daum2009gradient,
  title={Gradient estimation for particle flow induced by log-homotopy for nonlinear filters},
  author={F. Daum and J. Huang and A. Noushin and M. Krichman},
  booktitle={Proc. SPIE },
  volume={7336},
  pages={65--75},
  year={2009},
  month={Apr},
  organization={SPIE}
}

@inproceedings{daum2010exact,
  title={Exact particle flow for nonlinear filters},
  author={F. Daum and J. Huang and A. Noushin},
  booktitle={Proc. SPIE},
  volume={7697},
  pages={769704},
  year={2010},
  month={Apr}
}

@inproceedings{daum2013particle,
  title={Particle flow with non-zero diffusion for nonlinear filters},
  author={F. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={8745},
  pages={87450P},
  year={2013},
  month={May}
}

@inproceedings{daum2014seven,
  title={Seven dubious methods to mitigate stiffness in particle flow with non-zero diffusion for nonlinear filters, {Bayesian} decisions, and transport},
  author={F. Daum and J. Huang},
  booktitle={Proc. SPIE},
  volume={9092},
  pages={72--82},
  year={2014},
  month={May}
}

@inproceedings{li2015particle,
  title={Particle flow auxiliary particle filter},
  author={Y. Li and L. Zhao and M. J. Coates},
  booktitle={Proc. Comput. Adv. Multi-Sensor Adapt. Process.},
  pages={157--160},
  year={2015},
  month={Dec}
}

@inproceedings{7472424,
  author={Y. Li and L. Zhao and M. J. Coates},
  booktitle={Proc. Int. Conf. Acoust. Speech Signal Process.}, 
  title={Particle flow for particle filtering}, 
  year={2016},
  pages={3979-3983},
 }
 
 @inproceedings{ding2012implementation,
  title={Implementation of the {Daum-Huang} exact-flow particle filter},
  author={T. Ding and M. J. Coates},
  booktitle={Proc. IEEE Statist. Signal Process. Workshop},
  pages={257--260},
  year={2012}
}

@article{li2017particle,
  title={Particle filtering with invertible particle flow},
  author={Y. Li and M. J. Coates},
  journal={IEEE Trans. Signal Process.},
  volume={65},
  number={15},
  pages={4102--4116},
  year={2017},
  month={Aug}
}

@book{warner1983foundations,
  title={Foundations of differentiable manifolds and {Lie} groups},
  author={F. W. Warner},
  volume={94},
  year={1983},
  publisher={Springer Science \& Business Media}
}

@inproceedings{hlinka2011distributed,
  title={Distributed {Gaussian} particle filtering using likelihood consensus},
  author={O. Hlinka and O. Slu{\v{c}}iak and F. Hlawatsch and P. M. Djuri{\'c} and M. Rupp},
  booktitle={Proc. Int. Conf. Acoust. Speech Signal Process.},
  address={Prague, Czech Republic},
  pages={3756--3759},
  year={2011},
  month={May}
}

@article{schuhmacher2008consistent,
  title={A consistent metric for performance evaluation of multi-object filters},
  author={D. Schuhmacher and B. T. Vo and B. N. Vo},
  journal={IEEE Trans. Signal Process.},
  volume={56},
  number={8},
  pages={3447--3457},
  year={2008},
  month={Aug}
}

@article{zhu2010generalized,
  title={A generalized asymmetric {S}tudent-t distribution with application to financial econometrics},
  author={D. Zhu and J. W. Galbraith},
  journal={Journal of Econometrics},
  volume={157},
  number={2},
  pages={297--305},
  year={2010},
  month={Aug}
}

@inproceedings{khan2015improvements,
  title={Improvements in the implementation of log-homotopy based particle flow filters},
  author={M. A. Khan and M. Ulmke},
  booktitle={Proc. Int. Conf. Inf. Fusion},
  pages={74--81},
  year={2015}
}

@inproceedings{pal2019particle,
  title={Particle flow particle filter using {G}romov's method},
  author={S. Pal and M. J. Coates},
  booktitle={Proc. Comput. Adv. Multi-Sensor Adapt. Process.},
  pages={634--638},
  year={2019},
  month={Dec}
}

@inproceedings{daum2010exact1,
  title={Exact particle flow for nonlinear filters: seventeen dubious solutions to a first order linear underdetermined {PDE}},
  author={F. Daum and J. Huang},
  booktitle={Proc. Asilomar Conf. Signals, Syst. Comput},
  pages={64--71},
  year={2010},
  month={Nov}
}

@article{lee1994extended,
  title={Extended {Kalman} filter based nonlinear model predictive control},
  author={J. H. Lee and N. L. Ricker},
  journal={Industrial \& Engineering Chemistry Research},
  volume={33},
  number={6},
  pages={1530--1541},
  year={1994},
  month={Jun}
}

@article{wan2001unscented,
  title={The unscented {Kalman} filter},
  author={E. A. Wan and R. Van Der Merwe and S. Haykin},
  journal={Kalman filtering and neural networks},
  volume={5},
  number={2007},
  pages={221--280},
  year={2001},
}

@article{evensen2003ensemble,
  title={The ensemble {K}alman filter: Theoretical formulation and practical implementation},
  author={G. Evensen},
  journal={Ocean Dyn.},
  volume={53},
  number={4},
  pages={343--367},
  year={2003}
}

@inproceedings{julier1997new,
  title={New extension of the {Kalman} filter to nonlinear systems},
  author={Julier, Simon J and Uhlmann, Jeffrey K},
  booktitle={Proc. SPIE},
  volume={3068},
  pages={182--193},
  year={1997},
  month={Apr}
}
